Online learning with dynamics: A minimax perspective

We study the problem of online learning with dynamics, where a learner interacts with a stateful environment over multiple rounds. In each round of the interaction, the learner selects a policy to deploy and incurs a cost that depends on both the chosen policy and current state of the world. The state-evolution dynamics and the costs are allowed to be time-varying, in a possibly adversarial way. In this setting, we study the problem of minimizing policy regret and provide non-constructive upper bounds on the minimax rate for the problem. Our main results provide sufficient conditions for online learnability for this setup with corresponding rates. The rates are characterized by 1) a complexity term capturing the expressiveness of the underlying policy class under the dynamics of state change, and 2) a dynamics stability term measuring the deviation of the instantaneous loss from a certain counterfactual loss. Further, we provide matching lower bounds which show that both the complexity terms are indeed necessary. Our approach provides a unifying analysis that recovers regret bounds for several well studied problems including online learning with memory, online control of linear quadratic regulators, online Markov decision processes, and tracking adversarial targets. In addition, we show how our tools help obtain tight regret bounds for a new problems (with non-linear dynamics and non-convex losses) for which such bounds were not known prior to our work.

==> macros.tex <==
% \DeclareMathOperator*{\Ex}{\vphantom{p}\mathbb{E}}
% \let\inf\undef
% \DeclareMathOperator*{\inf}{\vphantom{p}inf}
% \let\sup\undef
% \DeclareMathOperator*{\sup}{\vphantom{p}sup}


%%%%%%%%%% NOTATION %%%%%%%%%%

\newcommand*{\wrench}{\includegraphics[scale=0.1]{graphics/wrench3}}%
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\muca}{\mu_{\scalebox{0.6}{\ensuremath{\mathcal A}}}}
\newcommand{\Constr}{\mathcal{C}}
\newcommand{\Las}{\mathcal{L}\mathrm{as}}
\newcommand{\trace}{\text{tr}}

\newcommand{\card}[1]{\ensuremath{\mbox{card}\left(#1\right)}}
\newcommand{\conv}[1]{\ensuremath{\mbox{conv}\left(#1\right)}}

\newcommand{\dham}{\text{d}_{\scalebox{0.6}{H}}}

\newcommand{\vcdim}[1]{\ensuremath{\text{vc}\left(#1\right)}}
\newcommand{\ldim}[1]{\ensuremath{\text{ldim}\left(#1\right)}}

% loss functions
%\newcommand\loss{\mathrm{loss}}
\newcommand\loss{\boldsymbol{\ell}}
\newcommand\hingeloss{\loss_{\text{hng}}}
\newcommand\ReLU{\text{ReLU}}

% Shortcuts
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\trm}[1]{\textrm{#1}}
\newcommand{\V}{\mc{V}}
\newcommand{\gap}{\mrm{gap}}
% General math
%\newcommand{\v}{\mbb{v}}
\newcommand{\pred}{\widehat{{y}}}
\newcommand{\predbf}{\widehat{\mathbf{y}}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\sign}{\mrm{sign}}
\newcommand{\argmin}[1]{\underset{#1}{\mrm{argmin}} \ }
\newcommand{\argmax}[1]{\underset{#1}{\mrm{argmax}} \ }
\newcommand{\reals}{\mathbb{R}}
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]} % brackets
\newcommand{\Ebr}[1]{\mathbb{E}\left\{ #1 \right\}} % curly braces
\newcommand{\En}{\mathbb{E}}  % no brackets or braces
\newcommand{\Eu}[1]{\underset{#1}{\mathbb{E}}}  % subscript no braces
\newcommand{\Ebar}{\Hat{\Hat{\mathbb{E}}}}  % no brackets or braces
\newcommand{\Esbar}[2]{\Hat{\Hat{\mathbb{E}}}_{#1}\left[ #2 \right]} % subscript + brackets
\newcommand{\Es}[2]{\mathbb{E}_{#1}\left[ #2 \right]} % subscript + brackets
\newcommand{\Ps}[2]{\mathbb{P}_{#1}\left[ #2 \right]}
\newcommand{\Prob}{\mathbb{P}}
%\newcommand{\conv}{\operatorname{conv}}
\newcommand{\inner}[1]{\left\langle #1 \right\rangle}
\newcommand{\ip}[2]{\left<#1,#2\right>}
\newcommand{\lv}{\left\|}
\newcommand{\rv}{\right\|}
\newcommand{\Phifunc}[1]{\Phi\left(#1\right)}
\newcommand{\ind}[1]{{\bf{1}}\left\{#1\right\}}
%\newcommand{\ind}[1]{\ 1\hspace{-2.3mm}{1}{\left\{#1\right\}}}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{T}}}}
\newcommand{\eqdist}{\stackrel{\text{d}}{=}}
\newcommand{\alphT}{\widehat{\alpha}(T)}
\newcommand{\PD}{\mathcal P}
\newcommand{\QD}{\mathcal Q}
\newcommand{\jp}{\ensuremath{\mathbf{p}}}
\newcommand{\brho}{{\boldsymbol{\rho}}}
\newcommand{\proj}{\text{Proj}}
\newcommand{\Eunderone}[1]{\underset{#1}{\En}}
\newcommand{\Eunder}[2]{\underset{\underset{#1}{#2}}{\En}}
\newcommand{\bphi}{\boldsymbol\phi}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\e}{\boldsymbol{e}}
% Bold symbols
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand\f{\mathbf{f}}
\renewcommand\v{\mathbf{v}}

%\newcommand{\xtree}{\scalebox{0.85}{\ensuremath{\mathsf{\overset{\text{\leafright}}{\boldsymbol{X}}}}}}
\newcommand{\xtree}{\scalebox{0.85}{\ensuremath{\mathsf{\boldsymbol{X}}}}}

% Calligraphic symbols
\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cE{\mathcal{E}}
\newcommand\cI{\mathcal{I}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cP{\mathcal{P}}
\newcommand\cS{\mathcal{S}}
\newcommand\cX{\mathcal{X}}
\newcommand\cY{\mathcal{Y}}
\newcommand\X{\mathcal{X}}
\newcommand\Y{\mathcal{Y}}
\newcommand\Z{\mathcal{Z}}
\newcommand\F{\mathcal{F}}
\newcommand\G{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\N{\mathcal{N}}
\newcommand\M{\mathcal{M}}
\newcommand\W{\mathcal{W}}

% Rademacher and Dudley
\newcommand\Rad{\mathscr{R}}
\newcommand{\CondRad}{\ensuremath{\widehat{\Rad}}}
\newcommand{\RadStat}{\ensuremath{\mathcal{R}}^{{iid}}}
\newcommand{\RadStatWorst}{\ensuremath{\widebar{\mathcal{R}}}^{{iid}}}
\newcommand{\CondRadStat}{\ensuremath{\widehat{\mathcal{R}}}^{{iid}}}
\newcommand{\RadSeq}{\ensuremath{\mathcal{R}}^{seq}}
\newcommand{\CondRadSeq}{\ensuremath{\widehat{\mathcal{R}}}^{{seq}}}
\newcommand{\CondDudleyStat}{\ensuremath{\widehat{\mathcal{D}}^{{iid}}}}
\newcommand{\DudSeq}{\ensuremath{\mathcal{D}}^{{seq}}}


\newcommand{\karthik}[1]{{\color{red} Karthik: #1}}
\newcommand{\sasha}[1]{{\color{blue} Sasha: #1}}

% Notations
%\newcommand\ldim{\mathrm{Ldim}}
%\newcommand\ldim{\mathrm{Sdim}}
\newcommand\fat{\mathrm{fat}}
\newcommand\Img{\mbox{Img}}
\newcommand\sparam{\sigma} % Strong convexity constant
\newcommand\Psimax{\ensuremath{\Psi_{\mathrm{max}}}}

% Calligraphic notations
\newcommand\Val{\mathcal{V}}
\newcommand\Valdet{\mathcal{V}^{\mathrm{det}}}
\newcommand\Dudley{\mathfrak{D}}
\newcommand\Reg{\mbf{Reg}}
\newcommand\D{\mbf{D}}
\renewcommand\P{\mbf{P}}

% For the examples section
\newcommand\Xcvx{\X_\mathrm{cvx}}
\newcommand\Xlin{\X_\mathrm{lin}}
\newcommand{\Relax}[3]{\mbf{Rel}_{#1}\left(#2 ~\middle| #3 \right)}
\newcommand{\Rel}{\mbf{Rel}}
\newcommand{\Relfull}[2]{\mbf{Rel}^{\dagger}_{#1}\left(#2 \right)}

\newcommand{\multiminimax}[1]{\ensuremath{\left\llangle #1\right\rrangle}}

\newcommand{\Fclass}[2]{\F_{#1}\boldsymbol{[}#2\boldsymbol{]}}
\newcommand{\constr}{{\mathscr{C}}}
\def\deq{\triangleq}

\newcommand{\OPT}{{\sf OPT}}
\newcommand{\SDP}{{\sf SDP}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\frameit}[1]{
    \begin{center}
    \framebox[1\columnwidth][c]{
        \begin{minipage}{.99\columnwidth}
        #1
		\vspace{-0mm}
        \end{minipage}
    }
    \end{center}
}

\newcommand{\Mhat}{{\widehat{\cM}}}

==> notation.tex <==
%!TEX root = paper.tex
\section*{Notation and Macros}
\begin{minipage}{0.6\textwidth}
\begin{center}
 \begin{tabular}{|c c c|}
 \hline
 Description & Macro & Symbol \\
 \hline
 Value of Game & \bs val & $\val$\\
 Generic Function Class & \bs Xg & $\Xg$\\
 Function Class & \bs F & $\F$\\
 Adversary Space & \bs Z & $\Z$\\
 State Space & \bs X & $\X$\\
 Action Space & \bs U & $\U$\\
 Generic Algorithm & \bs alg & $\alg$\\
 Loss Function & \bs loss & $\loss$\\
 Learner Policy &\bs f & $\f$\\
 State of system & \bs st & $\st$\\
 Action taken by learner &  \bs ac &  $\ac$\\
 Adversary Action & \bs z & $\z$\\
 Learner Distribution & \bs ld & $\ld$\\
 Adversary Distribution & \bs ad & $\ad$\\
 Dynamics function & \bs dyn & $\dyn$\\
 Time Horizon & \bs T & $\T$\\
 Regret & \bs reg & $\reg$\\
 Noise in Dynamics & \bs w & $\w$\\
 Noise distribution & \bs Dnoise & $\Dnoise$\\
 Loss Function (different) & \bs losst & $\losst$\\
 State explicit & \bs stf\{$t$\}\{$f_{1:t-1}$\} & $\stf{t}{f_{1:t-1}}$\\
 Sequential Rademacher & \bs Rseq & $\Rseq$\\
 Rademacher Variable & \bs rad & $\rad$\\
 Loss at Stationarity & \bs losss & $\losss$\\
 Mixability parameter & \bs stable & $\stable$\\
 Learner Dist Space & \bs distl & $\distl$\\
 Adversary Dist Space & \bs dista & $\dista$\\
 Regularization Function & \bs regf & $\regf$\\
 Regularization Parameter & \bs regp & $\regp$\\
 ERM (math mode) & \bs ERM & $\ERM$\\
 \hline
\end{tabular}
\end{center}
\end{minipage}
\begin{minipage}{0.4\textwidth}
  \begin{center}
   \begin{tabular}{|c c c|}
   \hline
   Description & Macro & Symbol \\
   \hline
   Real Number & \bs real & $\real$\\
   Trace of Matrix & \bs trace & $\trace$\\
   Composition & \bs com & $\com$\\
   Diagonal matrix & \bs diag & $\diag$\\
   \hline
  \end{tabular}
  \end{center}
  \begin{center}
   \begin{tabular}{|c c c|}
   \hline
   Description & Macro & Symbol \\
   \hline
   State Dimension & \bs sdim & $\sdim$\\
   Action dimension & \bs adim & $\adim$\\
   LQR Q matrix & \bs lqrQ & $\lqrQ$\\
   LQR R matrix & \bs lqrR & $\lqrR$\\
   LQR A matrix & \bs lqrA & $\lqrA$\\
   LQR B matrix & \bs lqrB & $\lqrB$\\
   Tracking norm bound & \bs zbnd & $\zbnd$\\
   Comparator class & \bs Ftrack & $\Ftrack$\\
   Policy Matrix & \bs K & $\K$\\
   Policy Bias & \bs bias & $\bias$\\
   K bound & \bs Kbnd & $\Kbnd$\\
   bias bound & \bs cbnd & $\cbnd$\\
   A+BK bound & \bs rholq & $\rholq$\\
   Effective bias M & \bs Meff & $\Meff$\\
   Value Function & \bs valf & $\valf$ \\
   Stability Kappa & \bs stk & $\stk$\\
   Stability Gamma & \bs stg & $\stg$\\
   Stability L & \bs lqL & $\lqL$\\
   Stability H & \bs lqH & $\lqH$\\
   Normal Distirbution & \bs N & $\N$\\
   Normal COvariance & \bs W & $\W$\\
   State Covariance & \bs cov & $\cov$\\
   \hline
  \end{tabular}
  \end{center}
  \begin{center}
   \begin{tabular}{|c c c|}
   \hline
   Description & Macro & Symbol \\
   \hline
   State Size & \bs ssize & $\ssize$\\
   Action Size & \bs asize & $\asize$\\
   Policy class MDP & \bs Fmdp & $\Fmdp$\\
   Transition Matrix & \bs trans & $\trans$\\
   MDP dist of states & \bs mdpd & $\mdpd$\\
   Mixing Time & \bs mixt & $\mixt$\\
   \hline
  \end{tabular}
  \end{center}
\end{minipage}

